Learning Neighborhood Representation from Multi-Modal Multi-Graph: Image, Text, Mobility Graph and Beyond

Recent urbanization has coincided with the enrichment of geotagged data, such as street view and point-of-interest (POI). Region embedding enhanced by the richer data modalities has enabled researchers and city administrators to understand the built environment, socioeconomics, and the dynamics of cities better. While some efforts have been made to simultaneously use multi-modal inputs, existing methods can be improved by incorporating different measures of 'proximity' in the same embedding space - leveraging not only the data that characterizes the regions (e.g., street view, local businesses pattern) but also those that depict the relationship between regions (e.g., trips, road network). To this end, we propose a novel approach to integrate multi-modal geotagged inputs as either node or edge features of a multi-graph based on their relations with the neighborhood region (e.g., tiles, census block, ZIP code region, etc.). We then learn the neighborhood representation based on a contrastive-sampling scheme from the multi-graph. Specifically, we use street view images and POI features to characterize neighborhoods (nodes) and use human mobility to characterize the relationship between neighborhoods (directed edges). We show the effectiveness of the proposed methods with quantitative downstream tasks as well as qualitative analysis of the embedding space: The embedding we trained outperforms the ones using only unimodal data as regional inputs.

==> table/asymmetrical.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{0.8\textwidth}{!}{%
    \begin{tabular}{l|c|c|c}
      \toprule
      Model & Poverty rate & Average household income & Employment rate\\ 
      \midrule
      Mean & - & - & -\\ 
      Concatenation & - & - & - \\
      Concatenation + PCA  & - & - & - \\
      \bottomrule
    \end{tabular}
    }
    \caption{Improved predication $R^2$ over baseline, with different approaches to combine $K$ and $Q$}
    \label{table:asymmetrical}
\end{table*}

==> table/demographics.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{1\textwidth}{!}{%
    \begin{tabular}{l|c|c|c|c|c|c}
      \toprule
    %   Model & Median Age & Year of Education & Percentage of White Population \\ 
    %   \midrule
    %   Urban2Vec \cite{wang2020urban2vec}& $0.326\pm0.056$ & $0.701\pm0.035$  & $0.472\pm0.052$ \\ 
    %   GAE \cite{DBLP:journals/corr/KipfW16}& $0.261\pm0.072$ & $0.672\pm0.024$ & $0.480\pm0.061$ \\ 
    %   \method DIST & $0.344\pm0.052$ & $0.756\pm0.030$ & $0.630\pm0.038$ \\
    %   \method MOB & $0.338\pm0.063$ & $0.780\pm0.020$ & $\mathbf{0.736\pm0.021}$\\
    %   \method DIST+MOB & $\mathbf{0.374\pm0.060}$ & $\mathbf{0.790\pm0.022}$ & $0.734\pm0.030$ \\
        Model & Median age & Years of education & Percentage of white population & Poverty rate & Average household income & Employment rate\\ 
      \midrule
      Urban2Vec \cite{wang2020urban2vec}& $0.326\pm0.056$ & $0.701\pm0.035$  & $0.472\pm0.052$ & $0.418\pm0.052$ & $0.515\pm0.052$ & $0.441\pm0.059$\\
      GAE \cite{DBLP:journals/corr/KipfW16}& $0.261\pm0.072$ & $0.672\pm0.024$ & $0.480\pm0.061$ & $0.432\pm0.078$& $0.457\pm0.047$ & $0.435\pm0.079$\\
      \method DIST & $0.344\pm0.052$ & $0.756\pm0.030$ & $0.630\pm0.038$ & $0.488\pm0.053$ & $0.548\pm0.047$ & $0.530\pm0.046$\\
      \method MOB & $0.338\pm0.063$ & $0.780\pm0.020$ & $\mathbf{0.736\pm0.021}$& $0.591\pm0.049$ & $0.616\pm0.029$ & $0.615\pm0.038$\\
      \method DIST+MOB & $\mathbf{0.374\pm0.060}$ & $\mathbf{0.790\pm0.022}$ & $0.734\pm0.030$ & $\mathbf{0.602\pm0.049}$ & $\mathbf{0.630\pm0.038}$ & $\mathbf{0.627\pm0.036}$\\
      \bottomrule
    \end{tabular}
    }
    \caption{Prediction $R^2$ on demographic and economic characteristics with linear regression model}
    \label{table:demographics}
\end{table*}

==> table/economics.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{0.68\textwidth}{!}{%
    \begin{tabular}{l|c|c|c}
      \toprule
      Model & Poverty Rate & Average Household Income & Employment Rate\\ 
      \midrule
      Urban2Vec \cite{wang2020urban2vec}& $0.418\pm0.052$ & $0.515\pm0.052$ & $0.441\pm0.059$\\ 
      GAE \cite{DBLP:journals/corr/KipfW16}& $0.432\pm0.078$& $0.457\pm0.047$ & $0.435\pm0.079$\\ 
      \method DIST & $0.488\pm0.053$ & $0.548\pm0.047$ & $0.530\pm0.046$\\
      \method MOB & $0.591\pm0.049$ & $0.616\pm0.029$ & $0.615\pm0.038$\\
      \method DIST+MOB & $\mathbf{0.602\pm0.049}$ & $\mathbf{0.630\pm0.038}$ & $\mathbf{0.627\pm0.036}$\\
      \bottomrule
    \end{tabular}
    }
    \caption{Prediction $R^2$ on Neighborhood Economic Characteristics with Linear Regression Model}
    \label{table:economics}
\end{table*}
